A Game-Theoretic Account of Responsibility Allocation

When designing or analyzing multi-agent systems, a fundamental problem is responsibility ascription: to specify which agents are responsible for the joint outcome of their behaviors and to which extent. We model strategic multi-agent interaction as an extensive form game of imperfect information and define notions of forward (prospective) and backward (retrospective) responsibility. Forward responsibility identifies the responsibility of a group of agents for an outcome along all possible plays, whereas backward responsibility identifies the responsibility along a given play. We further distinguish between strategic and causal backward responsibility, where the former captures the epistemic knowledge of players along a play, while the latter formalizes which players -- possibly unknowingly -- caused the outcome. A formal connection between forward and backward notions is established in the case of perfect recall. We further ascribe quantitative responsibility through cooperative game theory. We show through a number of examples that our approach encompasses several prior formal accounts of responsibility attribution.

==> not_backward_responsible.tex <==
	\node[scale=0.8, state] (In) {$s_0$};
	\node[scale=0.8, state, green] (2a) [below left = 1.2 and 1.2 of In] {$s_1$};
	\node[scale=0.8, state] (2b) [below right = 1.2 and 1.2 of In]{$s_2$};

	\node[scale=0.8, state] (t3) [below left = 1.2 and 0.7 of 2b]{$s_3$};
	\node[scale=0.8, state, red] (t4) [below right = 1.2 and 1.0 of 2b]{$s_4$};
	
	\node[scale=0.8, state, red] (f1) [below left = 1.2 and 0.7 of t3]{$s_5$};
	\node[scale=0.8, state, green] (f2) [below right = 1.2 and 0.7 of t3]{$s_6$};
	
	\draw (In) -- (2a) node[left, pos=0.5] {$a$};
	\draw (In) -- (2b) node[right, pos=0.5] {$b$};
	
	\draw (2b) -- (t3) node[left, pos=0.5] {$y$};
	\draw (2b) -- (t4) node[right, pos=0.5] {$z$};
	
	\draw (t3) -- (f1) node[left, pos=0.5] {$a$};
	\draw (t3) -- (f2) node[right, pos=0.5] {$b$};

	\draw [-, densely dashed] (In) -- (t3);
